Searching For Music Mixing Graphs: A Pruning Approach

Music mixing is compositional -- experts combine multiple audio processors to achieve a cohesive mix from dry source tracks. We propose a method to reverse engineer this process from the input and output audio. First, we create a mixing console that applies all available processors to every chain. Then, after the initial console parameter optimization, we alternate between removing redundant processors and fine-tuning. We achieve this through differentiable implementation of both processors and pruning. Consequently, we find a sparse mixing graph that achieves nearly identical matching quality of the full mixing console. We apply this procedure to dry-mix pairs from various datasets and collect graphs that also can be used to train neural networks for music mixing applications.

==> tables/console-ablation-more-metrics.tex <==
\begin{table*}
\setlength\tabcolsep{2.8pt}
\renewcommand{\arraystretch}{.8}
\begin{center}
\caption{
\it
Matching performances of the mixing consoles using different processor type configurations. 
%The strings, e.g., \texttt{ecnsgdr}, denote the processors used in the chain and their orders.
}
\vspace{-.5mm}
\begin{tabular}{lc|cccc|c|c|ccccc}
\toprule
 & & $L_\mathrm{a}$ & $L_\mathrm{lr}$ & $L_\mathrm{m}$ & $L_\mathrm{s}$  & FAD & SI-SDR & $\Delta$RMS & $\Delta$CR & $\Delta$SW & $\Delta$SI & $\Delta$Bark
\\ \midrule
\multicolumn{2}{l|}{Base graph (sum of dry sources)}
& $19.7$ & $1.52$ & $1.46$ & $74.3$ & $4.44$ & $-9.73$ & $\smash{1.79\times 10^{-2}}$ & $31.4$ & $\smash{5.27\times 10^{-2}}$ & $\smash{2.06\times 10^{-2}}$ & $172$\\
\midrule
+ Gain/panning 
& \texttt{\textcolor{white}{ecns\textcolor{black}{g}dr}}
& $.689$ & $.686$ & $.634$ & $.752$ & $1.26$ & $-8.11$ & $\smash{1.80\times 10^{-3}}$& $18.0$ & $\smash{1.95\times 10^{-2}}$ & $\smash{2.35\times 10^{-2}}$ & $.276$ \\
+ Stereo imager 
& \texttt{\textcolor{white}{ecn\textcolor{black}{sg}dr}}
& $.676$ & $.671$ & $.623$ & $.734$ & $1.23$ & $-7.69$ & $\smash{1.39\times 10^{-3}}$ & $17.7$ & $\smash{1.39\times 10^{-2}}$& $\smash{2.39\times 10^{-2}}$ & $.269$ \\
+ Equalizer 
& \texttt{\textcolor{white}{\textcolor{black}{e}cn\textcolor{black}{sg}dr}}
& $.557$ & $.549$ & $.493$ & $.637$ & $.900$ & $-6.78$ & $\smash{5.29\times 10^{-4}}$ & $2.39$ & $\smash{1.02\times 10^{-2}}$ & $\smash{1.77\times 10^{-2}}$ & $.087$\\
+ Reverb 
& \texttt{\textcolor{white}{\textcolor{black}{e}cn\textcolor{black}{sg}d\textcolor{black}{r}}}
& $.481$ & $.471$ & $.457$ & $.523$ & $.665$ & $-5.58$ & $\smash{3.36\times 10^{-4}}$ & $1.80$ & $\smash{9.01\times 10^{-3}}$ & $\smash{2.41\times 10^{-3}}$ & $.069$\\
+ Compressor 
& \texttt{\textcolor{white}{\textcolor{black}{ec}n\textcolor{black}{sg}d\textcolor{black}{r}}}
& $.423$ & $.407$ & $.385$ & $.492$ & $.504$ & $-4.94$ & $\smash{4.85\times 10^{-4}}$ & $1.94$ & $\smash{2.49\times 10^{-2}}$ & $\smash{2.44\times 10^{-3}}$ & $.088$ \\
+ Noisegate 
& \texttt{\textcolor{white}{\textcolor{black}{ecnsg}d\textcolor{black}{r}}}
& $.414$ & $.398$ & $.375$ & $.485$ & $.463$ & $-4.55$ & $\smash{2.36\times 10^{-4}}$ & $1.61$ & $\smash{9.00\times 10^{-3}}$ & $\smash{1.70\times 10^{-3}}$ & $.085$ \\
\midrule
+ Multitap delay (full) 
& \texttt{\textcolor{white}{\textcolor{black}{ecnsgdr}}}
& $.409$ & $.395$ & $.375$ & $.469$ & $.458$ & $-4.50$ & $\smash{3.05\times 10^{-4}}$ & $1.34$ & $\smash{8.56\times 10^{-3}}$ & $\smash{2.23\times 10^{-3}}$ & $.095$ \\
%\midrule
%Consistency check 
%& \texttt{\textcolor{white}{\textcolor{black}{ecnsgdr}}}
%\\ 
\bottomrule
\end{tabular}

\label{table:mixing-console}
\end{center}
\vspace{-5mm}
\end{table*}

